Compact-Table: Efficiently Filtering Table Constraints with Reversible Sparse Bit-Sets

In this paper, we describe Compact-Table (CT), a bitwise algorithm to enforce Generalized Arc Consistency (GAC) on table con- straints. Although this algorithm is the default propagator for table constraints in or-tools and OscaR, two publicly available CP solvers, it has never been described so far. Importantly, CT has been recently improved further with the introduction of residues, resetting operations and a data-structure called reversible sparse bit-set, used to maintain tables of supports (following the idea of tabular reduction): tuples are invalidated incrementally on value removals by means of bit-set operations. The experimentation that we have conducted with OscaR shows that CT outperforms state-of-the-art algorithms STR2, STR3, GAC4R, MDD4R and AC5-TC on standard benchmarks.

==> compact-table - copie/figures/initmasks.tex <==
\begin{figure}
\centering
\begin{subfigure}[b]{0.4\textwidth}
\centering
\begin{tabular}{|c|c|c|c|}
\hline 
\textbf{T} & $x$ & $y$ & $z$ \\ 
\hline 
0 & a & a & a \\ 
\hline 
1 & a & a & b \\ 
\hline 
2 & a & b & c \\ 
\hline 
3 & b & a & a \\ 
\hline 
\rowcolor{gray!40}
 & a & c & b \\ 
\hline 
4 & a & b & b \\ 
\hline 
5 & b & a & b \\ 
\hline 
6 & b & b & a \\ 
\hline 
7 & b & b & b \\ 
\hline 
\end{tabular} 
\caption{The indexed tuples}
\end{subfigure}
\begin{subfigure}[b]{0.59\textwidth}
\centering
\begin{tabular}{r|c|c|c|c|c|c|c|c|}
\cline{2-9}
$\f{currTable}$ & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ 
\cline{2-9} 
$\f{supports}[x,a]$ & 1 & 1 & 1 & 0 & 1 & 0 & 0 & 0 \\ 
\cline{2-9}
$\f{supports}[x,b]$ & 0 & 0 & 0 & 1 & 0 & 1 & 1 & 1 \\ 
\cline{2-9} 
$\f{supports}[y,a]$ & 1 & 1 & 0 & 1 & 0 & 1 & 0 & 0 \\ 
\cline{2-9}
$\f{supports}[y,b]$ & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 1 \\ 
\cline{2-9} 
$\f{supports}[y,d]$ & \cellcolor{gray!40}{0} & \cellcolor{gray!40}{0} & \cellcolor{gray!40}{0} & \cellcolor{gray!40}{0} & \cellcolor{gray!40}{0} & \cellcolor{gray!40}{0} & \cellcolor{gray!40}{0} & \cellcolor{gray!40}{0} \\ 
\cline{2-9} 
$\f{supports}[z,a]$ & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 \\ 
\cline{2-9}
$\f{supports}[z,b]$ & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 1 \\ 
\cline{2-9}
$\f{supports}[z,c]$ & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 
\cline{2-9}
\end{tabular} 
\caption{The corresponding bit-sets}
\end{subfigure}
\caption{Illustration of the data structures after the initialization of $\langle x,y,z \rangle \in T$. The tuple $(a, c, b)$ will not be indexed and $d$ will be removed from $dom(y)$.\label{fig:initmasks}}
\end{figure}
